Confidence-Controlled Exploration: Efficient Sparse-Reward Policy Learning for Robot Navigation

Reinforcement learning (RL) is a promising approach for robotic navigation, allowing robots to learn through trial and error. However, real-world robotic tasks often suffer from sparse rewards, leading to inefficient exploration and suboptimal policies due to sample inefficiency of RL. In this work, we introduce Confidence-Controlled Exploration (CCE), a novel method that improves sample efficiency in RL-based robotic navigation without modifying the reward function. Unlike existing approaches, such as entropy regularization and reward shaping, which can introduce instability by altering rewards, CCE dynamically adjusts trajectory length based on policy entropy. Specifically, it shortens trajectories when uncertainty is high to enhance exploration and extends them when confidence is high to prioritize exploitation. CCE is a principled and practical solution inspired by a theoretical connection between policy entropy and gradient estimation. It integrates seamlessly with on-policy and off-policy RL methods and requires minimal modifications. We validate CCE across REINFORCE, PPO, and SAC in both simulated and real-world navigation tasks. CCE outperforms fixed-trajectory and entropy-regularized baselines, achieving an 18\% higher success rate, 20-38\% shorter paths, and 9.32\% lower elevation costs under a fixed training sample budget. Finally, we deploy CCE on a Clearpath Husky robot, demonstrating its effectiveness in complex outdoor environments.

==> 2_related_work.tex <==
\section{Related Work}
\label{section:related_work}


Learning-based approaches, in particular DRL have pushed the boundaries of mobile robot navigation for unstructured and dynamically changing environments~\cite{sathyamoorthy2022terrapn,weerakoon2021terp,liang2022adaptiveon}. Nevertheless, these methods suffer from sample efficiency under sparse rewards settings because dense rewards play an important role in learning for DRL methods. We summarize the related work next.  

\textbf{Outdoor Robot Navigation:} Navigation, path planning and obstacle avoidance are extensively-studied fundamental research problems in the field of robotics \cite{planning_review,motion_planning_survey}. Number of deterministic~\cite{dijkstra1959note,fox1997dwa} and stochastic~\cite{kuffner2000rrt,kavraki1996probabilistic} algorithms have been proposed in the past three decades. However, robot navigation in complex outdoor environments still remains a challenging problem given the complexity and diversity of the setting.  
% Classical approaches used in outdoor robot navigation utilize techniques such as feature classification \cite{pan2020feature_classification}, semantic segmentation \cite{guan2021ganav}, and potential fields \cite{chiang2015potential_fields} to represent terrain traversability. However, such methods are significantly biased towards human annotation \cite{wigness2019rugd}. 
%
To perform robot-centric decision-making, deep reinforcement learning (DRL) strategies have been employed in recent studies for outdoor navigation \cite{zhou2021review,shah2021ving}. 
For example, deterministic policies such as DDPG\cite{weerakoon2021terp}, A3C\cite{zhang2018uneven_a3c}, and DQN\cite{josef2020deep_dqn_rainbow}  with dense rewards have been incorporated for robot navigation on uneven terrains.
\invis{For example, in \cite{josef2020deep_dqn_rainbow}, a DQN network with rainbow architecture is proposed to locally navigate a robot on simulated rough terrains using zero-range to local range elevation sensing. An A3C architecture based DRL network is utilized in \cite{zhang2018uneven_a3c} to determine optimal actions for robot navigation in simulated uneven terrains. The method proposed in~\cite{weerakoon2021terp} uses DDPG to train an end-to end DRL network with attention to extract intermediate elevation features for navigation costmap generation.} An adaptive model that directly learns control and environmental dynamics is presented in~\cite{liang2022adaptiveon}. Moreover, segmentation\cite{guan2021ganav} and self supervised~\cite{sathyamoorthy2022terrapn} methods for identifying navigable regions have also been utilized with a combination of DRL based navigation methods to ensure stable and efficient navigation. 

% On the other hand the surface properties are possible to learn through self-supervised methods~\cite{sathyamoorthy2022terrapn}. To address the limitation of the predefined characteristics of the traversability of a region that is associated with the specific type of robot, 

% \ncomment{Can someone put references here from the heavy tailed policy paper lit review?}

\textbf{Sparse Reward Settings:} In sparse reward settings, an environment rarely produces a useful reward which significantly affects the reinforcement policy leaning \cite{zai2020sparse_reward_definition}. To deal with this issue, several reward shaping methods based on intrinsic curiosity and information gain-based shaping have been proposed~\cite{hussein2017reward_shaping}. For example, reward shaping based methods such as \cite{botteghi2020reward_shaping,houthooft2016vime_reward_shaping} encourage the agent to explore unvisited states by modifying the actual reward output. However, such approaches require additional effort and expertise in reward function design. Imitation learning and learning from demonstration methods are another approach for dealing with sparse rewards in practice~\cite{nair2018overcoming_demonstrations}. \invis{For example,in methods \cite{nair2018overcoming_demonstrations}, rewards corresponding to an expert's actions are extracted using inverse reinforcement learning based imitation learning techniques. Learning from expert demonstrations with replay buffers is also employed to improve policy convergence.} However, obtaining reliable expert demonstrations for continuous control tasks is practically infeasible and challenging~\cite{ravichandar2020recent,vecerik2017leveraging_sparse_reward}.
%

\textbf{Heavy-tailed Policy Parametrization:} The possibility of incorporating heavy-tailed distributions to RL tasks is theoretically analyzed in recent literature \cite{bedi_chakraborty_ht, sparse_reward_souradip}. For example, in \cite{chou2017beta}, beta distribution is utilized with dense rewards for stochastic policy training to enhance the state exploration capabilities. Further, a heavy-tailed policy gradient method is proposed in \cite{bedi_chakraborty_ht} to find convergence to global maxima while minimizing the risk of local maxima convergence. Inspired by these ideas, we propose a heavy-tailed adaptive reinforce algorithm to deal with sparse rewards in complex outdoor environments.

==> macros.tex <==
%\usepackage{xcolor}
%\usepackage{amssymb}
%\usepackage{graphicx}
% \usepackage{subfigure}
%\usepackage{mathtools}
%\usepackage{amsmath}
%\usepackage{gensymb}


==> sections/Alternative_Introduction.tex <==
\section{Introduction}

\begin{wrapfigure}{r}{0.4\textwidth}
  \centering
  \includegraphics[width=0.37\textwidth]{figures/noobssamples.png}
  \caption{\textcolor{red}{TODO: NEED A DETAILED CAPTION THAT CLEARLY HIGHGLIGHTS THE BENEFITS OF YOUR APPROACH}}
  \label{fig:teaser}
\end{wrapfigure} 

Reinforcement learning (RL) \cite{sutton2018reinforcement} is an important component of learning in robotic systems in a wide variety of complex domains, including search-and-rescue, disaster relief, and planetary exploration applications \cite{bajece781162, murphy2014disaster, SCHILLING199883}. However, reward function sparsity \cite{vecerik2017leveraging_sparse_reward} and non-stationarity frequently arise when applying RL methods to robotics problems, which can result in policy optimization schemes being sample inefficient in practice. This issue is especially important in robotic systems, due to the simulation-intensive nature of RL methods and the computationally expensive nature of simulation of realistic robotics platforms. Attempts to reduce the computational burden of RL methods applied to robotics have been made through assuming access to expert demonstrations \cite{vecerik2017leveraging_sparse_reward, nair2018overcoming_demonstrations}, but this does not reduce the transient errors in policy gradient estimates. This is due to the fact that both reward sparsity and changing system dynamics induced by the evolution of policies during training cause biases in policy evaluation errors that are not easily overcome in practice.
%
% In this paper, we develop methods that are attuned to transience in transitions as a proxy for reward sparsity, since there does not exist any way to estimate reward sparsity
%
In this paper, we address the problem of reward sparsity by developing a new adaptive trajectory length selection scheme for policy gradient methods that is attuned to the non-stationarity induced by policy evolution during training.

%In most real-world applications, however, a reward function specifying the task to be performed must first be handcrafted, which often results in reward sparsity, i.e., the reward takes  non-zero values at only small subset of possible states -- is a practical necessity, as it is typically intractable for problem designers to handcraft dense rewards \cite{vecerik2017leveraging_sparse_reward}. Additionally, due to the simulation-intensive nature of RL methods and the computationally expensive nature of simulation of realistic robotics platforms, ensuring sample efficiency of new methods is a critical issue that must be addressed. Indeed, the moment we must deal with sparse rewards, we enter into a complicated regime of intelligently balancing the need to expend samples to acquire reward information with the need to limit the overall number of samples needed to achieve the end goal. This balancing act instantiates the well-known exploration-exploitation trade-off in RL.

Effective methods for policy optimization in the presence of non-stationarity typically tune their learning rates (step-sizes) to some measure of drift or volatility, such as the variance of a gradient estimator, as in AdaGrad \citep{duchi2011}. However, the sample variance of a gradient estimator alone is insufficient to capture transient effects and reward sparsity, as this is a function of the transition model itself. Unfortunately, standard approaches to analyzing the sample complexity of reinforcement learning (RL) methods \cite{kakade2003sample, lattimore2013sample, dann2015sample} and especially policy gradient (PG) methods \cite{kumar2019sample}, do not characterize the effect of reward sparsity or transient transitions on sample complexity, leaving little to go on. How then might one go about addressing this issue for these standard PG schemes? Starting with this simple base case is well-motivated, since any insights that improve their performance can naturally be applied to more sophisticated PG methods like TRPO and PPO \cite{schulman2015trust, schulman2017proximal}.
%
%
%
%
% THIS PARAGRAPH GIVES A BACKGROUND OF THE PROBLEM AND PRIOR WORK. DO NOT TALK ABOUT YOUR WORK HERE.  Instead, we propose an alternate statistic to attune policy evaluation trajectory lengths based on the theory of Markov chain mixing times \citep{}. This specification departs from standard approaches to analyzing the sample complexity gradient (PG) method, whose foundational results on sample complexity \cite{kakade2003sample, lattimore2013sample, dann2015sample} and especially for policy gradient (PG) methods \cite{kumar2019sample} do not characterize the effect of reward sparsity or transient transitions on sample complexity. As illustrated empirically in Figure \ref{fig:teaser} IF THIS IS PRIOR PART, DO NOT PUT THAT ON PAGE 1, BUT RATHER ON PAGE 3, the classic actor-critic \cite{Konda2000} algorithm exhibits sample inefficiency in the presence of sparse rewards, due to the implied transience/bias in value function estimates. How might one go about addressing this issue for these standard PG schemes? Starting with this simple base case is well-motivated, since any insights that improve their performance can naturally be applied to more sophisticated PG methods like TRPO and PPO \cite{schulman2015trust, schulman2017proximal}.

A salient feature of REINFORCE and related PG methods is the trajectory length, or the number of samples collected from the environment before each gradient update is performed. Despite its obvious influence on sample complexity through its direct, multiplicative effect on total samples consumed and its powerful yet more subtle effect on gradient estimation quality and convergence, the choice of trajectory length is largely overlooked in the literature. Indeed, it is typically assumed to be a user-specified hyperparameter in need of tuning. The following question arises: is it possible to adaptively select trajectory length based on the task at hand in order to improve overall sample complexity? Recent work on PG methods under Markovian sampling \cite{suttlemixing2023} reveals that mixing times -- the time it takes for a given Markov chain to approximately converge to its steady-state distribution -- can be used to determine optimal trajectory length. Mixing times are typically difficult to estimate, however, so an alternative route is required. 

\noindent {\bf Main Results:} In this work, we propose an alternative, easy-to-use statistic to adaptively tune policy evaluation trajectory lengths: the Shannon entropy of the policy being evaluated. To motivate this novel approach, we establish an empirical connection between policy entropy and mixing time. We do so by examining the relationship between policy entropy and the spectral gap of the induced Markov chain transition matrices on toy examples with known transition kernels. We find policy entropy and spectral gap to be positively correlated, suggesting that mixing time increases as entropy decreases. We then leverage this connection to develop our primary algorithmic contribution: a tractable, adaptive trajectory length selection scheme for policy gradient methods, called Ada-NAV, in which trajectory length is a decreasing function of policy entropy. We empirically demonstrate that our approach enjoys improved sample complexity as well as comparable or superior performance over fixed- and random-length trajectory schemes on a variety of robotics navigation tasks.

Our main contributions are as follows:
\begin{itemize}
    \item We empirically identify a novel connection between policy entropy and mixing time by examining the correlation between a policy's entropy and the spectral gap of the transition matrix of its induced Markov chain.
    %
    \item We propose a novel mapping between policy entropy and trajectory length that facilitates exploration in sparse-reward environments and provides the basis of our adaptive trajectory length scheme for PG methods, called Ada-NAV.
    %
    \item We provide empirical results in goal-reaching navigation tasks illustrating that Ada-NAV is more sample efficient than both constant trajectory length and randomly sampled trajectory length schemes. To increase problem complexity, we consider tasks with obstacles and uneven terrain.
    %
    \item We evaluate the navigation performance of Ada-NAV in both simulated and real-world complex outdoor environments using a Clearpath Husky robot. We observe that, for a fixed sample budget, Ada-NAV leads to x\% increase in navigation success rate, y\% decrease in the navigation path length, and z\% decrease in the elevation cost compared to the policies obtained by the other methods.
    
\end{itemize}

WHAT ARE THE BENEFITS OF YOUR APPROACH? HOW DID YOU TEST AND EVALUATE> GIVE QUALITATIVE AND QUANTITATIVE METRICS

==> sections/theory.tex <==
\section{Theoretical Justifications} 

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\columnwidth]{figures/cheeger.png}
    \caption{Cheeger inequality. Will replace image with latex code if we use this for the paper.}
    \label{fig:cheeger}
\end{figure}

\textcolor{red}{Need to show that with any policy, $\pi$, the induced Markov Chain $P(s'|s)$ is reversible with following assumptions: 1)if the transition kernel $P(s'|s,a)$ is deterministic and 2) there exists $n$ actions to go from state $i$ to state $j$ iff there exists $n$ actions to go from state $i$ to state $j$ then}

\textcolor{red}{An Markov chain is reversible if it's ergodic, which we always assume, and if for states $i, j$: $\mu(i)P(j|i) = \mu(j)P(j|i)$ where $\mu$ is the stationary distribution}
